Reducing Order Enforcement Cost in Complex Query Plans

Algorithms that exploit sort orders are widely used to implement joins, grouping, duplicate elimination and other set operations. Query optimizers traditionally deal with sort orders by using the notion of interesting orders. The number of interesting orders is unfortunately factorial in the number of participating attributes. Optimizer implementations use heuristics to prune the number of interesting orders, but the quality of the heuristics is unclear. Increasingly complex decision support queries and increasing use of covering indices, which provide multiple alternative sort orders for relations, motivate us to better address the problem of optimization with interesting orders. We show that even a simplified version of optimization with sort orders is NP-hard and provide principled heuristics for choosing interesting orders. We have implemented the proposed techniques in a Volcano-style cost-based optimizer, and our performance study shows significant improvements in estimated cost. We also executed our plans on a widely used commercial database system, and on PostgreSQL, and found that actual execution times for our plans were significantly better than for plans generated by those systems in several cases.

==> texfiles/ack.tex <==
\subsection*{Acknowledgments}
\paper{
\small{
\noindent The {\em NP-hardness} result and 2-approximation are joint work with 
Ajit A. Diwan and Ch. Sobhan Babu. We thank C. Santosh Kumar for 
implementing the extensions to external sorting in Postgres.
}
}
\techreport{
\noindent The {\em NP-hardness} result and 2-approximation are joint work with 
Prof. Ajit A. Diwan and Ch. Sobhan Babu. We thank C. Santosh Kumar for 
implementing the extensions to external sorting in PostgreSQL.
}



==> texfiles/techrep_section1.tex <==
\Section{Introduction} 
\label{sec:intro}
Algorithms that exploit sort orders are widely used to
implement joins, grouping, duplicate elimination and other set operations.
Query optimizers traditionally deal with sort orders by using 
the notion of interesting orders.
\eat{
The number of interesting orders is unfortunately factorial in the number of 
%participating attributes.
Optimizer implementations use heuristics to prune 
the number of interesting orders, but the quality of the heuristics is unclear.
Increasingly complex decision support queries
and increasing use of covering indices\footnote{{\em i.e.,} 
indices containing all attributes of the relation that are used in the query}, 
which provide multiple alternative
sort orders for relations, motivate us to better address the problem
of optimization with interesting orders.
}
\eat{
We show that even a simplified version of optimization
with sort orders is NP-hard and provide principled heuristics
for choosing interesting orders. 
We have implemented the proposed techniques in a Volcano-style 
cost-based optimizer, and our performance study shows significant
improvements in estimated cost.  
We also executed our plans on a widely used commercial database system, 
and on PostgreSQL, and found that actual execution times for our
plans were significantly better than for plans generated by those systems
in several cases.
}
\eat{
Decision support queries, extract-transform-load (ETL) 
operations, data cleansing and integration often use complex joins, aggregation,
set operations and duplicate elimination. 
Sorting based query processing algorithms 
for these operations are well known. Sorting based algorithms
are quite attractive when physical sort orders of one or more base relations 
fulfill the sort order requirements of operators either completely or partially.
Further, secondary indices that cover a query\footnote{{\em i.e.,} 
contain all attributes of the relation that are used in the query} 
are being increasingly used in read-mostly environments. 
Query covering indices
make it very efficient to obtain desired sort orders without accessing 
the data pages. These factors make it possible for sort based plans to 
significantly outperform hash based counterparts. 
}
The notion of interesting orders~\cite{SEL:SIGMOD79} has allowed optimizers to consider
plans that could be locally sub-optimal, but produce orders that are
beneficial for other operators, and thus produce a better plan overall.
However, the number of interesting orders for most operators is factorial
in the number of attributes involved. 
%This is not acceptable as queries 
%in the afore mentioned applications do contain large number of attributes 
%in joins and set operations. 
Malkemus et.al.~\cite{MALK:SIGMOD96} 
identify this problem and propose an approach of using a flexible order 
specification to reduce the number of interesting orders for certain
operations, such as grouping, which can work with any sort order on
the input. However, their approach works only for single input operators. 
Sorting based algorithms for binary operators 
such as join and union,
though agnostic to the exact input order, require a matching order from multiple
inputs, which makes the problem harder to solve. 
In this report we address the problem of optimization with interesting
sort orders.  We make the following technical contributions:

\begin{enumerate}
\item Often order requirements of operators are partially satisfied by 
inputs. For instance, consider a merge-join with join predicate
$(r.c_1=s.c_1$ {\em and} $r.c_2=s.c_2)$. A clustering index on $r.c_1$ (or on
$r.c_2$ or $s.c_1$ or $s.c_2$) is helpful in getting the
desired order efficiently; a secondary index that covers the query has
the same effect. 
%Partial sort orders, when exploited 
%properly, can yield benefits by avoiding run-generation I/O 
%of external sort. 

We highlight (in \refsec{sec:pso}) the need for exploiting partial sort orders and 
show how a minor modification to the standard
replacement selection algorithm can avoid run generation I/O completely
when input is known to have a partial sort order. Further, we
extend a cost-based optimizer to take into account partial sort
orders.

\item We consider 
%(in Sections~\ref{sec:nphard} and \ref{sec:ford}) 
operators with flexible order requirements and 
address the problem of choosing good
interesting orders so that complete or partial sort orders already available
from inputs can be exploited. 
\begin{itemize}
    \item In Sections~\ref{sec:nphard} we show that a special case of
    finding optimal sort orders is NP-hard and give a 2-approximation
    algorithm to choose interesting sort orders for a join tree.
    \item In \refsec{sec:ford} we address a more general case of the 
    problem. In many cases, the knowledge of indices and available 
    physical operators in the system allows us to narrow down the 
    search space to a small set of orders.  We formalize this idea (in 
    \refsec{subsec:favord}) through 
    the notion of {\em favorable orders}, and propose a heuristic to 
    efficiently enumerate a small set of promising sort orders.
    Unlike heuristics used in optimizer implementations,
    our approach takes into account issues such as $(i)$ added choices of sort orders 
    for base relations due to the use of query covering indices 
    $(ii)$ sort orders that partially match an order requirement 
    $(iii)$ requirement of same sort order from multiple inputs 
    ({\em e.g.,} merge based join, union) and 
    $(iv)$ common attributes between multiple joins, grouping and set operations.
    
    In \refsec{subsec:optext} we also show how to integrate our extensions
    into a cost-based optimizer.
\end{itemize}

\item We present experimental results (in \refsec{sec:perf})
evaluating the benefits of the proposed
techniques. We compare the plans generated by our optimizer with those of 
three widely used database systems and show significant benefits
due to each of our optimizations.
\end{enumerate}


